SpecWatch: A Framework for Adversarial Spectrum Monitoring with Unknown Statistics

In cognitive radio networks (CRNs), dynamic spectrum access has been proposed to improve the spectrum utilization, but it also generates spectrum misuse problems. One common solution to these problems is to deploy monitors to detect misbehaviors on certain channel. However, in multi-channel CRNs, it is very costly to deploy monitors on every channel. With a limited number of monitors, we have to decide which channels to monitor. In addition, we need to determine how long to monitor each channel and in which order to monitor, because switching channels incurs costs. Moreover, the information about the misuse behavior is not available a priori. To answer those questions, we model the spectrum monitoring problem as an adversarial multi-armed bandit problem with switching costs (MAB-SC), propose an effective framework, and design two online algorithms, SpecWatch-II and SpecWatch-III, based on the same framework. To evaluate the algorithms, we use weak regret, i.e., the performance difference between the solution of our algorithm and optimal (fixed) solution in hindsight, as the metric. We prove that the expected weak regret of SpecWatch-II is O(T^{2/3}), where T is the time horizon. Whereas, the actual weak regret of SpecWatch-III is O(T^{2/3}) with probability 1 - {\delta}, for any {\delta} in (0, 1). Both algorithms guarantee the upper bounds matching the lower bound of the general adversarial MAB- SC problem. Therefore, they are all asymptotically optimal.

==> acknowledgement.tex <==
\section*{Acknowledgment}
The authors would like to thank...

==> algo.tex <==
\section{Monitoring Algorithms and Performance Analysis}
To answer those questions, we design four effective online algorithms, {\algA}, {\algB}, {\algC} and {\algD}.
%
In {\algA}, we select strategies based on monitoring history, and repeat the same strategy for certain timeslots to reduce switching costs.
%
%
Whereas, in {\algB}, we select strategies more strategically to improve the performance. We also rigorously bound the weak regrets of both algorithms. 
%CITEOURS
%Due to space limitation, all proofs are omitted and can be found in~\cite{OURS}.
To further reduce the weak regrets, we leverage the convenience of loss model in {\algC} and {\algD} and put more weight on exploitation than exploration.

\subsection{Design Rationale}
Both {\algA} and {\algB} are based on the batching version of exponential-weight algorithm for exploration and exploitation, where the idea of batching is inspired by \cite{arora2012online}.
%which is inspired by \cite{arora2012online}, where they use the idea of batching to calculate policy regret from weak regret. In our paper, we use this idea to limit switching costs. 
Our algorithms work as follows: The timeslots $1, 2, \ldots, T$ are grouped into consecutive and disjoint batches of size $\tau$.  The set of batches is $\mathcal{J} = \left\{ 1, 2, \ldots, j, \ldots, J\right\}$, where $J = \lceil T / \tau \rceil$. Let $t_j = (j-1)\tau$, then the $j$-th batch starts from timeslot $t_j + 1$ and ends at timeslot $t_j + \tau$ as shown in Fig.~\ref{fig:batch}. In both algorithms, strategies are selected according to their weights. Within each batch, the chosen strategy remains the same. At the end of each batch, strategy weights are updated according to the strategy reward or loss. 
%\vspace{-.2in}
The main notations are summarized in Table~\ref{tab:notation}.


\begin{figure}[ht!] %\label{fig:batch}
	\centering
	\includegraphics[width = 0.48\textwidth]{pics.pdf}	
	\caption{Example of batching timeslots with batch size $\tau=4$}
	\label{fig:batch}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%    table of notations
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%f

\setlength{\extrarowheight}{5pt}
\begin{table}[t!]
	\centering
	\caption{\textsc{Algorithm Notations}}
	\label{tab:notation}
	\begin{tabular}{ l  l}
		\toprule 
		%$r$         & unit reward of a single channel in a single timeslot
		%\\
		$f_{k, t}$  & actual channel reward of channel $k$ in timeslot $t$
		\\ 
		$g_{s, t}$  & actual strategy reward of strategy $s$ in timeslot $t$
		\\
		$\ell_{k, t}$ & actual channel loss of channel $k$ in timeslot $t$
		\\ 
		$y_{s, t}$  & actual strategy loss of strategy $s$ in timeslot $t$
		\\
		\arrayrulecolor{gray}\hline
		$\mathsf{f}_{k, j}$
		& actual channel reward of channel $k$ in batch $j$
		\\
		$\mathsf{g}_{s, j} =  \sum_{k \in s} \mathsf{f}_{k, j}$
		& actual strategy reward of strategy $s$ in batch $j$
		\\
		$\bar{\mathsf{f}}_{k, j}$
		& average channel reward of channel $k$ in batch $j$
		\\ 
		$\bar{\mathsf{g}}_{s, j} =  \sum_{k \in s} \bar{\mathsf{f}}_{k, j}$
		& average strategy reward of strategy $s$ in batch $j$
		\\
		$\bar{\mathsf{f}}^{\prime}_{k, j}$
		& virtual channel reward of channel $k$ in batch $j$
		\\
		$\bar{\mathsf{g}}^{\prime}_{s, j} =  \sum_{k \in s} \bar{\mathsf{f}}^{\prime}_{k, j}$
		& virtual strategy reward of strategy $s$ in batch $j$
		\\ 
		$\mathsf{l}_{k, j}$
		& actual channel loss of channel $k$ in batch $j$
		\\
		$\mathsf{y}_{s, j} =  \sum_{k \in s} \mathsf{l}_{k, j}$
		& actual strategy loss of strategy $s$ in batch $j$
		\\
		$\bar{\mathsf{l}}_{k, j}$
		& average channel loss of channel $k$ in batch $j$
		\\ 
		$\bar{\mathsf{y}}_{s, j} =  \sum_{k \in s} \bar{\mathsf{l}}_{k, j}$
		& average strategy loss of strategy $s$ in batch $j$
		\\
		$\bar{\mathsf{l}}^{\prime}_{k, j}$
		& virtual channel loss of channel $k$ in batch $j$
		\\
		$\bar{\mathsf{y}}^{\prime}_{s, j} =  \sum_{k \in s} \bar{\mathsf{l}}^{\prime}_{k, j}$
		& virtual strategy loss of strategy $s$ in batch $j$
		\\ 
		$\mathsf{h}_{k, j}$ 
		& channel weight of channel $k$ in batch $j$
		\\ 
		$\mathsf{w}_{s, j} =  \prod_{k \in s} \mathsf{h}_{k, j}$
		& strategy weight of strategy $s$ in batch $j$
		\\ 
		$\mathsf{W}_j = \sum_{s \in \mathcal{S}} \mathsf{w}_{s, j}$
		& total weight of all strategies in batch $j$
		\\ 
		$\mathsf{q}_{k, j}$
		%		$\mathsf{q}_{k, j} = \sum_{s: k \in s} \mathsf{p}_{s, j}$
		& channel probability of channel $k$ in batch $j$
		\\
		$\mathsf{p}_{s, j}$
		& strategy probability of strategy $s$ in batch $j$		
		\\
		\arrayrulecolor{black}\bottomrule	
		%$\bar{\mathsf{G}}_{{\algAabr}} \myeq \sum_{j = 1}^{J}\bar{\mathsf{g}}_{Z_j, j}$
	\end{tabular}
\end{table}



==> algoA.tex <==
\subsection{{\algA}}\label{ssec: algA}

\subsubsection{Algorithm Design}
{\algA} takes two parameters $\gamma$ and $\tau$ as input, where $\gamma$ is used to calculate strategy probability and update strategy weights. 
The strategy probabilities  are linear functions of strategy weights. The strategy weights are updated using an increasing function of rewards gained previously.

%It calculates strategy probabilities linear to strategy weights and updates the strategy weights according to rewards gained previously.

\textbf{Calculating Strategy Probability $\mathsf{p}_{s, j}$.}
%
%At the beginning of  batch $j$, 
We calculate the the probability of choosing strategy $s \in \mathcal{S}$ using
\begin{equation}
\label{eq: strategy prob}
\mathsf{p}_{s, j} = (1-\gamma)\frac{\mathsf{w}_{s, j}}{\mathsf{W}_j} + \frac{\gamma}{S},
\end{equation}
where $\gamma \in (0, 1)$ is a parameter, $\mathsf{w}_{s, j}$ is the strategy weight of strategy $s$ in batch $j$, and $\mathsf{W}_j = \sum_{s \in \mathcal{S}} \mathsf{w}_{s, j}$. It is a weighted average of two terms, where the first is to exploit strategies with good reward history, and the second guarantees the exploration over all strategies. $\gamma$ controls the balance between them. 

\textbf{Choosing Strategy $Z_j$ and Monitoring Spectrum.}
%At the beginning of each batch, w
We select a strategy $Z_j \in \mathcal{S}$ randomly according to the probabilities calculated above. The monitor keeps using $Z_j$ for all $\tau$ timeslots in batch $j$, i.e., $X_{[j] + i} = Z_j$ for $1 \leq i \leq \tau $. Therefore, the monitor only incurs switching cost $c (Z_{j-1}, Z_j)$ once for the whole batch $j$. 

Depending on the misuse behavior of MUs (discussed in Section~\ref{sec: model}), the monitor receives rewards on monitored channels accordingly. The monitor keeps record of $f_{k, [j] + i}$ for all  $k \in Z_j$ and $1 \leq i \leq \tau$. The strategy reward gained by the monitor is the summation of rewards over all monitored channels. 

%Specifically, let $\mathsf{f}_{k, j}$ be the total actual reward of channel $k$ throughout batch $j$, i.e.,
%\begin{equation}
%\label{eq: channel reward}
%\mathsf{f}_{k, j}= \sum_{i = 1}^{\tau} f_{k, [j] + i},
%\end{equation}
%where $f_{k, [j] + i}$ is either $r$ or 0 as defined in~\eqref{eq: reward r};
%then the strategy reward $\mathsf{g}_{Z_j,j}$ of strategy $Z_j$ throughout batch $j$ is 
%\begin{equation}
%\label{eq: strategy reward}		
%\mathsf{g}_{Z_j,j} = \sum_{k \in Z_j} \mathsf{f}_{k, j} = \sum_{k \in Z_j} \sum_{i = 1}^{\tau} f_{k, [j] + i}.
%\end{equation}


\textbf{Updating Strategy Weight $w_{s, j+1}$.}
At the end of each batch, we update strategy weights in the following steps.

%First, we calculate the average channel reward of each monitored channel $k \in Z_j$ in batch $j$,
First, we calculate the average channel reward of each channel $k \in \mathcal{K}$ in batch $j$,
%
\begin{equation}
\label{eq: average channel reward}
\bar{\mathsf{f}}_{k, j}= \frac{1}{\tau}\sum_{i = 1}^{\tau} f_{k, [j] + i}.
\end{equation}
%
By \eqref{eq: reward r}, $ \bar{\mathsf{f}}_{k, j} \in [0, r]$. 
%
We also calculate the probability of choosing channel $k \in Z_j$ by summing up the probabilities of strategies containing that channel,
\begin{equation}
\label{eq: channel probability}
\mathsf{q}_{k, j} = \sum_{s: k \in s} \mathsf{p}_{s, j}.
\end{equation}
where $s: k \in s$ denotes any strategy $s$ containing channel $k$.
%{\color{red} which is guaranteed to $\in \left[0,1 \right]$ since $\mathsf{q}_{k, j} = \sum_{s: k \in s} \mathsf{p}_{s, j} \leq \sum_{s \in \mathcal{S}} \mathsf{p}_{s, j} =1$, not sure we need to show this}
Based on~\eqref{eq: average channel reward} and~\eqref{eq: channel probability}, we calculate the \textit{virtual channel reward},
\begin{equation}
\label{eq: virtual channel reward}
\bar{\mathsf{f}}^{\prime}_{k, j} = \frac{\bar{\mathsf{f}}_{k, j}}{\mathsf{q}_{k,j}}.
\end{equation}

Then we update each \textit{channel weight} by %by multiplying it with an exponential function of virtual channel reward,
\begin{equation}
\label{eq: channel weight}
\mathsf{h}_{k, j+1} = \mathsf{h}_{k, j} 
\exp 
\left(
\gamma \bar{\mathsf{f}}^{\prime}_{k, j} / S
\right),
\end{equation}
where  $\mathsf{h}_{k, 1} = 1$ for all $k \in \mathcal{K}$.
Note that using virtual channel rewards instead of average channel rewards compensates the rewards of channels with low probabilities. Among the channels receiving rewards, those with lower probabilities can obtain higher virtual channel rewards, and therefore higher channel weights.

Finally, we give the formal definition of \textit{strategy weight}, which is defined as % the production of corresponding channel weights:
\begin{equation}
\label{eq: strategy weight}
\mathsf{w}_{s, j} \myeq  \prod_{k \in s} \mathsf{h}_{k, j}.
\end{equation}
Combining~\eqref{eq: channel weight} and~\eqref{eq: strategy weight}, we can directly update the strategy weight for each $s \in \mathcal{S}$ by
\begin{equation}
\label{eq: weight update}			
\mathsf{w}_{s, j+1} = \mathsf{w}_{s, j} \exp (\gamma \bar{\mathsf{g}}^{\prime}_{s, j} / S),
\end{equation}
where $\bar{\mathsf{g}}^{\prime}_{s, j}$ is the \textit{virtual strategy reward} for each  $s \in \mathcal{S}$, i.e., $$\bar{\mathsf{g}}^{\prime}_{s, j} = \sum_{k \in s} \bar{\mathsf{f}}^{\prime}_{k, j}.$$
Note that by combining~\eqref{eq: average channel reward},~\eqref{eq: channel probability} and~\eqref{eq: virtual channel reward}, we can directly calculate $\bar{\mathsf{g}}^{\prime}_{s, j}$ directly by
\begin{equation}
\nonumber
\label{eq: virtual strategy reward}
\bar{\mathsf{g}}^{\prime}_{s, j} 
= \sum_{k \in s} \bar{\mathsf{f}}^{\prime}_{k, j} 
= \sum_{k \in s} \frac{\bar{\mathsf{f}}_{k, j}}{\mathsf{q}_{k,j}}
= \sum_{k \in s} \frac{\frac{1}{\tau} \sum_{i = 1}^{\tau} f_{k, [j] + i}}{\sum_{s: k \in s}\mathsf{p}_{s,j}}.
\end{equation}

\noindent \textit{Remark.} We do not update strategy weights based on strategy rewards, but instead calculate channel weights~\eqref{eq: channel weight} first. This is because the rewards of monitored channels provide useful information on those \textit{unchosen strategies} containing these channels. 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%    Performance Analysis
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsubsection{Performance Analysis}\label{sssec:SW analysis}
%We skip the analysis of {\algA} due to page limit. We directly provide Theorem~\ref{thm1} to show that the expected weak regret of {\algA} is bounded. 
%%To analyze the performance of {\algA}, we first bound the difference between the reward achieved by {\algA} and that by best fixed algorithm (Lemma~\ref{lemma1}), and then prove the bound of the expected weak regret (Theorem~\ref{thm1}). 
%%
%More details can be found in~\cite{li2016specwatch}.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%    theorem 
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{theorem}
	\label{thm1}
	The expected weak regret of {\algA} is $O(T^{\frac{2}{3}})$ with parameters $\gamma = A_\gamma T^{-\frac{1}{3}} \in \left(0, 1\right)  \text{ and } \tau =  A_\tau T^{\frac{1}{3}} \in \left[1, T\right],$ where $A_\gamma$ and $A_\tau$ are constants. Specifically, 
	\begin{equation*}
	\Expect\left[R_{{\algAabr}}\right] 
	\leq
	\left((e-1)A_\gamma + \frac{A_\tau S\ln S}{A_\gamma} + \frac{1}{A_\tau}\right) T^{\frac{2}{3}}.
	\end{equation*}
\end{theorem}

Note that the coefficient of the bound is not a convex function of $A_\tau$ and $A_\tau$, therefore finding the optimal parameters is challenging. 
For better understanding of Theorem \ref{thm1}, we present a specific bound obtained by a particular choice of parameters $\gamma$ and $\tau$ in Corollary~\ref{coro1}.
%finding the optimal choice of parameters is challenging because it is depending on the real values of $C$, $K$, $S$, as well as the confidence level $1-\delta$. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%    corollary
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{corollary}
	\label{coro1}
	When $T \geq (e-1) S \ln S$, with parameters
	$\gamma = \sqrt[3]{\frac{S\ln S}{(e-1)^2T}}$
	and
	$\tau = \sqrt[3]{\frac{T}{(e-1)S\ln S}}$,
%	\begin{equation*}	
%	\gamma = \sqrt[3]{\frac{S\ln S}{(e-1)^2T}}
%	\quad \text{ and } \quad 
%	\tau = \sqrt[3]{\frac{T}{(e-1)S\ln S}},
%	\end{equation*}
	the expected weak regret of {\algA} is
	\begin{equation*}
	\Expect\left[R_{{\algAabr}}\right] 
	\leq
	3\left((e-1)S\ln S\right)^{\frac{1}{3}} T^{\frac{2}{3}}.
	\end{equation*}
\end{corollary}


\noindent \textit{Remark.} The expected weak regret of {\algA} is bounded by $O(T^{2/3})$. This upper bound matches the lower bound of the MAB-SC problem proved in~\cite{dekel2014bandits} which is used to model the {\problemName} in this paper. Thus, {\algA} is asymptotically optimal. If we calculate the normalized weak regret $\frac{R_{\algAabr}}{T}$, i.e., amortizing the regret to every timeslot, then it is clear that the expected value of normalized weak regret converges to 0 as $T$ approaches to $\infty$.


==> algoD.tex <==
\subsection{{\algD}}\label{ssec: algD}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%    algorithm SpecWatch-N+
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Like how we improve {\algA}, we can improve {\algB} by leveraging the loss model and change the way to update strategy weights. Here we introduce {\algD} as the upgraded version of {\algB}.


\subsubsection{Algorithm Design}
%$\mathsf{p}_{s, j} = (1-\gamma)\frac{\mathsf{w}_{s, j}}{\mathsf{W}_j} + \frac{\gamma}{S}$
%
%$\mathsf{w}_{s, j+1} = \mathsf{w}_{s, j} \exp (\gamma
%%			 \bar{\mathsf{g}}^{\prime}_{s, j}
%\sum_{k \in s} \frac{\frac{1}{\tau} \sum_{i = 1}^{\tau} f_{k, [j] + i}}{\sum_{s: k \in s}\mathsf{p}_{s,j}}
%/ S)$
%
%The pseudo-code of {\algD} is illustrated in Algorithm~\ref{SpecWatchN+}. The basic three phases remain the same as before. We only modify virtual channel loss calculation and channel weight calculation.

{\algD} takes the same four parameters $\tau$, $\gamma$, $\beta$ and $\eta$ as {\algC}, but $\beta$ is used to calculate virtual channel loss instead of virtual channel reward.
%
{\algD} also uses the same equation
%$\mathsf{p}_{s, j} = (1-\gamma)\frac{\mathsf{w}_{s, j}}{\mathsf{W}_j} + \frac{\gamma}{C}$, 
to calculate strategy probabilities. However, {\algD} uses the loss to update strategy weights 
%$\mathsf{w}_{s, j+1} = \mathsf{w}_{s, j} \exp (-\eta \bar{\mathsf{y}}^{\prime}_{s, j})$
like {\algB},
though the calculation of virtual channel losses
%$\bar{\mathsf{y}}^{\prime}_{s, j}$ 
is different.
% from that of {\algB}.


\textbf{Calculating Strategy Probability $\mathsf{p}_{s, j}$.} 
Same as {\algC}.

\textbf{Choosing Strategy $Z_j$ and Monitoring Spectrum.}
Same as {\algB}.

\textbf{Updating Strategy Weight $w_{s, j+1}$.}
We will use the virtual channel loss defined below to update the channel weights:
%\begin{equation*}
$
\bar{\mathsf{l}}^{\prime}_{k, j} 
=
\frac{ \bar{\mathsf{l}}_{k, j} - \beta}{{\mathsf{q}_
		{k,j}}}.
$
%= \frac{1/l}{{\mathsf{q}_
%		{k,j}}} - \bar{\mathsf{f}}^{\prime}_{k, j}  
%\begin{cases}
%\frac{ \bar{\mathsf{l}}_{k, j} + \beta}{{\mathsf{q}_
%		{k,j}}} \qquad &\mbox{if } k \in Z_j,\\
%\frac{1/l + \beta}{{\mathsf{q}_{k,j}}} \qquad &\mbox{otherwise.}
%\end{cases}		
%\end{equation*}		
Note that we set $\beta \in (0, \frac{1}{l} - r)$ in this algorithm, and thus $\bar{\mathsf{l}}^{\prime}_{k, j} $ is always positive.
%In {\algB}, however, the virtual reward of such a channel is $\frac{\bar{\beta}}{\mathsf{q}_{k,j}}$. 
%The parameter $\beta$ 


Then the channel weight of $k$ is updated by
\begin{equation}
\label{eq: channel weight in N +}
\mathsf{h}_{k, j+1} = \mathsf{h}_{k, j} 
\exp 
\left(
-\eta \bar{\mathsf{l}}^{\prime}_{k, j-1}
\right),
\end{equation}
where $\mathsf{h}_{k, 1} = 1$ for all $k \in \mathcal{K}$.
Thus, the strategy weight of $s$ is updated by using 
\begin{equation}
\label{eq： weight update in N+}			
\mathsf{w}_{s, j+1} = \mathsf{w}_{s, j} \exp (-\eta \bar{\mathsf{y}}^{\prime}_{s, j}),
\end{equation}
where the virtual strategy loss of $s$ is $\bar{\mathsf{y}}^{\prime}_{s, j}  = \sum_{k \in s}\bar{\mathsf{l}}^{\prime}_{k, j}$ and can be calculated directly by
\begin{equation}\label{eq: virtual strategy reward in N+}
\bar{\mathsf{y}}^{\prime}_{s, j} 
= \sum_{k \in s}
 \frac
 {\frac{1}{\tau}\sum_{i = 1}^{\tau} \ell_{k, [j] + i} - \beta}
 {(1-\gamma)\frac{\sum_{s: k \in s}\mathsf{w}_{s, j}}
	{\mathsf{W}_j} + \frac{\gamma C_k}{C}}  .
\end{equation}	


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%    Performance Analysis
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsubsection{Performance Analysis}
%%We analyze {\algD} with a similar approach as for {\algB}. 
%We first present two lemmas (Lemma~\ref{chernoff bound N+} and Lemma~\ref{SW-N+ reward}) to analyze losses, then we consider the switching costs and claim the upper bound of weak regret in Theorem~\ref{SW-N+ theorem}. We also provide a specific choice of parameters and show the resulting bound in Corollary~\ref{SW-N+ special}.
%
%Similar to \eqref{eq: cumu str loss}, 
%we first define the cumulative average loss of {\algD} to be 
%%\begin{equation*}
%$
%\bar{\mathsf{Y}}_{{\algDabr}} \myeq \sum_{j = 1}^{J}\bar{\mathsf{y}}_{Z_j, j},
%$
%%\end{equation*}
%where $Z_1, Z_2, \ldots, Z_J$ is strategy sequence generated by {\algD}. Then we have
%%\begin{equation*}
%$
%\mathsf{Y}_{{\algDabr}} = \tau \bar{\mathsf{Y}}_{{\algDabr}}.
%$
%%\label{eq: algoN+ batch}
%%\end{equation*} 
%
%For the ease of our remaining analysis, we further introduce the following notations,
%\begin{align}
%\bar{\mathsf{L}}_{k, n} \myeq \sum _{j =1}^{n} \bar{\mathsf{l}}_{k, j} 
%\quad &\mbox{and} \quad
%\bar{\mathsf{L}}^{\prime}_{k, n} \myeq \sum _{j =1}^{n} \bar{\mathsf{l}}^{\prime}_{k, j} 
%\quad \mbox{for} \quad k \in \mathcal{K},
%\\
%\bar{\mathsf{Y}}_{s, n} \myeq \sum _{j =1}^{n} \bar{\mathsf{y}}_{s, j} 
%\quad &\mbox{and} \quad
%\bar{\mathsf{Y}}^{\prime}_{s, n} \myeq \sum _{j =1}^{n} \bar{\mathsf{y}}^{\prime}_{s, j} 
%\quad \mbox{for} \quad s \in \mathcal{S},
%\end{align}
%where $n$ is an arbitrary batch index.
%%
%Then we have
%\begin{lemma}
%	\label{chernoff bound N+}
%	For any $\delta \in (0, 1)$, $\beta \in (0, \frac{1}{l} - r))$ and $k \in \mathcal{K}$ in {\algB}, we have
%	\begin{equation}
%	\Probability \left[
%	\bar{\mathsf{L}}^{\prime}_{k, n}
%	\geq 
%	\bar{\mathsf{L}}_{k, n}  
%	+ \sum_{j=1}^{n}\frac{1/l}{\mathsf{q}_{k, n}}
%	+ \frac{1}{\beta} \ln \frac{K}{\delta}
%	- \frac{n}{l}
%	\right] 
%	\leq
%	\frac{\delta}{K}.
%	\end{equation}
%\end{lemma}
%%The proof of this lemma is shown in Appendix. %~\ref{lemma5 proof}.
%
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%
%
%Next, we bound the difference between the cumulative strategy loss of {\algD} and that of the best fixed algorithm. 
%%The proof of this lemma is also shown in Appendix. %~\ref{lemma6 proof}.
%\begin{lemma}\label{SW-N+ reward}
%	For any type of adversaries, any $T > 0$, $\tau \in \left[1, T\right]$, $\beta \in (0, \frac{1}{l} - r))$, $\gamma = \frac{2lC}{2lC + K -l}$ and $0 < \eta < \frac{2}{2lC + K -l}$, we have 
%	\begin{equation*}
%	 \bar{\mathsf{Y}}_{\algBabr} - \bar{\mathsf{Y}}_{best}
%	\leq
%	\frac{2l}{\beta}\ln\frac{K}{\delta} + \frac{2 \ln S}{\eta} + \beta KJ.
%	\end{equation*}	
%	with probability at least $1-\delta$ for any $\delta \in (0,1)$.
%\end{lemma}
%
%
%
%Taking the the bound of switching costs, \eqref{eq: switching cost bound},  into consideration, we now bound the weak regret of {\algD}.
\begin{theorem}
	\label{SW-N+ theorem}
	With probability at least $1-\delta$, the weak regret of {\algB} is bounded by  $O(T^{\frac{2}{3}})$. In particular, choosing
	$tau = B_{\tau} T^{\frac{1}{3}} \in \left[1, T\right],$
	$\gamma =  \frac{2lC}{2lC + K -l},$
	$\beta = B_{\beta} T^{-\frac{1}{3}} \in \left(0, \frac{1}{l} - r\right),$
	$\text{and } \eta  = B_{\eta} T^{-\frac{1}{3}} \in (0, \frac{2}{2lC + K -l})$,
%	\begin{align*}
%	\tau &= B_{\tau} T^{1/3} \in \left[1, T\right],\\
%	\gamma &=  {2lC}/{(2lC + K -l)},\\
%	\beta &= B_{\beta} T^{-1/3} \in \left(0, 1/l - r\right),\\
%	\text{and } \quad \eta  &= B_{\eta} T^{-1/3} \in (0, 2/{(2lC + K -l)}),
%	\end{align*}	
	where $ B_{\tau}$, $B_{\gamma}$, $B_{\beta}$ and $B_{\eta}$ are constants, 
	we have
	\begin{align}
	\nonumber
	R_{\algDabr}
	\leq 
	\left(
	B_{\beta}K
	+
	\frac{2lB_{\tau}}{B_{\beta}} \ln \frac{K}{\delta}		
	+ \frac{2\ln S B_{\tau}}{{B_\eta}}
	+ \frac{1}{B_{\tau}}
	\right) T^{\frac{2}{3}}.
	\end{align}
\end{theorem}
%\begin{proof}
%	\begin{align*}
%%	&
%	R_{\algDabr}
%%	\\	
%	=~& 
%	Y_{{\algDabr}} + L_{{\algDabr}}
%	-	Y_{best} - L_{best} 
%	\\
%	\leq~&
%	Y_{{\algDabr}} - Y_{best} + J
%	\\
%	=~&
%	 \tau (\bar{\mathsf{Y}}_{\algDabr} - \bar{\mathsf{Y}}_{best} )
%	+ \frac{T}{\tau}
%	\\
%	\leq~&
%	\tau
%	\left(
%%\frac{2JC}{\gamma}
%%+
%\frac{2l}{\beta} \ln \frac{K}{\delta}		
%+ \frac{2\ln S }{\eta}
%+ JK\beta
%	\right)	
%	+ \frac{T}{\tau},
%	\\
%	=~&	
%%	\left(
%%	\frac{2C}{\gamma}  
%%	+ 
%	\beta K	
%%	\right) 
%	T	
%	+
%	\tau
%	\left(
%	\frac{2l}{\beta} \ln \frac{K}{\delta}		
%	+ \frac{2\ln S }{\eta}
%	\right)	
%	+ 
%	\frac{T}{\tau},
%%	\stepcounter{equation}\tag{\theequation}\label{eq: N+ eq}
%	\end{align*}
%	with probability at least $1- \delta$.
%%	The last inequality follows from Lemma \ref{SW+ reward}. 
%	Plugging in the values of parameters finishes the proof. 
%\end{proof}

%We now give an example choice of parameters to reach a specific bound. 
\begin{corollary}\label{SW-N+ special}
	Under the condition of 	
	\begin{equation}
	T \geq \max \left\{
	B, 
	\frac{(2lC + K - l )^3 (\ln S)^3  }{B^2}
	\right\},	
	\label{eq: + condition N+}
	\end{equation}
	using parameters
	$\tau = B^{-\frac{1}{3}} T^{\frac{1}{3}}$,
	$\gamma = \frac{2lC}{2lC + K -l}$,
	$\beta =   \frac{1}{K} B^{\frac{1}{3}} T^{-\frac{1}{3}}$,
	and $\eta  = 2\ln S B^{-\frac{2}{3}} T^{-\frac{1}{3}}$,
%	\begin{align*}
%	\tau &= B^{-1/3} T^{1/3},\\
%	\gamma &= {2lC}/{(2lC + K -l)},\\
%	\beta &=   B^{1/3} T^{-1/3}/K,\\
%	\text{and } \quad \eta  &= 2\ln S B^{-2/3} T^{-1/3},
%	\end{align*}
	where $B = 2{lK\ln\frac{K}{\delta}}$, we have
	\begin{equation}
	R_{\algDabr}
	\leq
	4\left(2{lK\ln\frac{K}{\delta}}\right)^{\frac{1}{3}} T^{\frac{2}{3}},
	\end{equation}
	with probability at least $1-\delta$.
\end{corollary}



==> biography.tex <==
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Ming}}]{Ming Li}
	received the B.S. degree in geochemistry
	from Peking University, Beijing, China,
	in 2009 and the M.S. degree in computer science
	from Colorado School of Mines, Golden, CO,
	USA, in 2015.
	She is currently working toward the Ph.D. degree
	at Colorado School of Mines. Her main
	research interests include game theory, contract
	theory, crowdsourcing, smartphone-based sensing
	systems, visible light communication technologies.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{DJ}}]{Dejun Yang}
	is the Ben L. Fryrear Assistant Professor of Computer Science at Colorado School of Mines. He received his PhD degree in computer science from Arizona State University in 2013 and BS degree in computer science from Peking University, Beijing, China, in 2007. 
	
	His research interests include economic and optimization approaches to networks, crowdsourcing, smart grid, and security and privacy. 
	
	He received Best Paper Awards at {IEEE GLOBECOM'2015}, {IEEE MASS'2011}, {ICC'2011, 2012}, and a Best Paper Award Runner-up at {IEEE ICNP'2010}. He also served as a TPC member for many conferences including IEEE INFOCOM, ICC and GLOBECOM.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Jian}}]{Jian Lin}
	is a PhD candidate of Computer Science at Colorado School of Mines. He received his Master and BS degree in computer science from Southwest Jiaotong University, Chengdu China, in 2014 and 2011, respectively. His research interests include economic and optimization approaches to networks, crowdsensing and mobile computing.
\end{IEEEbiography}

\begin{IEEEbiography}{Ming Li}
	Biography text here.
\end{IEEEbiography}

\begin{IEEEbiography}{Jian Tang}
	Biography text here.
\end{IEEEbiography}
